The Renormalized Yukawa Hamiltonian: Spectrum, Parton Distribution Functions, and Resource Estimates for Quantum Simulation

We apply the Renormalization Group Procedure for Effective Particles (RGPEP) to the front form Yukawa Hamiltonian, yielding a renormalized (effective) Hamiltonian, accurate up to second order in the coupling strength. Subsequently, we examine the spectrum and parton distribution functions produced by the renormalized Hamiltonian, and show that the addition of counterterms leads to finite results. Resource estimates for quantum simulation are calculated for a single `Ladder Operator Block Encoding' (LOBE), and show that the cost to block encode the renormalized Hamiltonian is comparable to block encoding the bare Hamiltonian.

==> macros.tex <==
\newcommand{\twopartdef}[3]
{
	\left\{
		\begin{array}{lll}
			#1 & \mbox{if } #2 \\
			#3 & \mbox{otherwise } 
		\end{array}
	\right.
}
\newcommand{\Soln}{\noindent{\bf Solution}}
\newcommand{\csch}{{\rm csch}}
\newcommand{\sech}{{\rm sech}}
\newcommand{\T}{(Townsend)~}
\newcommand{\In}{Individual:~}
\newcommand{\G}{Group:~}
\newcommand{\NC}{{\bf Extra information not required for credit:}~}
\newcommand{\TP}{{\bf Total:}~}
\newcommand{\PO}{{\bf (1 Point)}~}
\newcommand{\PT}{{\bf (2 Points)}~}
\newcommand{\PTh}{{\bf (3 Points)}~}
\newcommand{\PF}{{\bf (4 Points)}~}
\newcommand{\PFi}{{\bf (5 Points)}~}
\newcommand{\PS}{{\bf (6 Points)}~}
\newcommand{\PSe}{{\bf (7 Points)}~}
\newcommand{\PE}{{\bf (8 Points)}~}
\newcommand{\PN}{{\bf (9 Points)}~}
\newcommand{\PTe}{{\bf (10 Points)}~}
\newcommand{\PEl}{{\bf (11 Points)}~}
\newcommand{\PTwe}{{\bf (12 Points)}~}
\newcommand{\PThi}{{\bf (13 Points)}~}
\newcommand{\PFo}{{\bf (14 Points)}~}
\newcommand{\PFif}{{\bf (15 Points)}~}
\newcommand{\PSi}{{\bf (16 Points)}~}
\newcommand{\RP}{{\bf Relevant problems:}~}
\newcommand{\AP}{{\bf Assigned problems:}~}
\def\ket#1{\left\vert #1 \right\rangle}
\def\bra#1{\left\langle #1 \right\vert}
\def\braket#1#2{\left\langle #1 \vert #2\right\rangle}
\newcommand{\kpz}{\ket{+{\bfz}}}
\newcommand{\kmz}{\ket{-{\bfz}}}
\newcommand{\bpz}{\bra{+{\bfz}}}
\newcommand{\bmz}{\bra{-{\bfz}}}
\newcommand{\kpx}{\ket{+{\bfx}}}
\newcommand{\kmx}{\ket{-{\bfx}}}
\newcommand{\bpx}{\bra{+{\bfx}}}
\newcommand{\bmx}{\bra{-{\bfx}}}
\newcommand{\kpy}{\ket{+{\bfy}}}
\newcommand{\kmy}{\ket{-{\bfy}}}
\newcommand{\bpy}{\bra{+{\bfy}}}
\newcommand{\bmy}{\bra{-{\bfy}}}
\newcommand{\be}{\begin{equation}}
\newcommand{\ee}{\end{equation}}
\newcommand{\bp}{\begin{pmatrix}}
\newcommand{\ep}{\end{pmatrix}}
\newcommand{\ben}{\begin{enumerate}}
\newcommand{\een}{\end{enumerate}}
\newcommand{\px}{\bp0&1\\1&0\ep}
\newcommand{\py}{\bp0&-i\\i&0\ep}
\newcommand{\pz}{\bp1&0\\0&-1\ep}
\newcommand{\id}{\bp1&0\\0&1\ep}
\newcommand{\pxpx}{\bp0&0&0&1\\0&0&1&0\\0&1&0&0\\1&0&0&0\ep}
\newcommand{\pypy}{\bp0&0&0&-1\\0&0&1&0\\0&1&0&0\\ -1&0&0&0\ep}
\newcommand{\pzpz}{\bp1&0&0&0\\0&-1&0&0\\0&0&-1&0\\0&0&0&1\ep}
\newcommand{\emf}{{\cal E}}
\newcommand{\bfE}{{\bf E}}
\newcommand{\bfB}{{\bf B}}
\newcommand{\bfn}{{\bf n}}
\newcommand{\bfdl}{{\bf dl}}
\newcommand{\bfdA}{{\bf dA}}
\newcommand{\bfp}{{\bf p}}
\newcommand{\bfr}{{\bf r}}
\newcommand{\bfi}{{\bf i}}
\newcommand{\bfj}{{\bf j}}
\newcommand{\bfk}{{\bf k}}
\newcommand{\iot}{i\omega t}
\newcommand{\eiot}{e^{i\omega t}}
\newcommand{\bfe}{{\bf e}}
\newcommand{\bfc}{{\bf c}}
\newcommand{\bfcj}{\bfc_j}
\newcommand{\cja}{c_{j\alpha}}
\newcommand{\cjb}{c_{j\beta}}
\newcommand{\cjc}{c_{jP}}
\newcommand{\cjd}{c_{j\delta}}
\newcommand{\bfu}{{\bf u}}
\newcommand{\bfv}{{\bf v}}
\newcommand{\bfN}{{\bf N}}
\newcommand{\bfx}{{\bf x}}
\newcommand{\bfy}{{\bf y}}
\newcommand{\bfz}{{\bf z}}
\newcommand{\bfZ}{{\bf Z}}
\newcommand{\Neq}{{N^{\mbox{\scriptsize eq}}}}
\newcommand{\dt}{{\Delta t}}
\newcommand{\bfbeta}{{\mbox{\boldmath $\beta$}}}
\newcommand{\bfzero}{{\mbox{\boldmath $0$}}}
\newcommand{\bfone}{{\mbox{\boldmath $1$}}}
\newcommand{\bfnabla}{{\mbox{\boldmath $\nabla$}}}
\newcommand{\LamInv}{{\mbox{$\Lambda^{-1}$}}}
\newcommand{\LamInvT}{{\mbox{$\Lambda^{-1}$}^T}}
\newcommand{\taumin}{{\tau_{\mbox{\tiny $\min$}}}}
\newcommand{\rhoomb}{{\frac{\rho}{mb}}}
\newcommand{\phip}{{\phi'\left(\rhoomb\right)}}
\newcommand{\phipp}{{\phi''\left(\rhoomb\right)}}
\newcommand{\phipx}{{\phi'\left(x\right)}}
\newcommand{\phippx}{{\phi''\left(x\right)}}
\newcommand{\vl}{{\vec{\ell}}}

